5G Wings: Investigating 5G-Connected Drones Performance in Non-Urban Areas

Unmanned aerial vehicles (UAVs) have become extremely popular for both military and civilian applications due to their ease of deployment, cost-effectiveness, high maneuverability, and availability. Both applications, however, need reliable communication for command and control (C2) and/or data transmission. Utilizing commercial cellular networks for drone communication can enable beyond visual line of sight (BVLOS) operation, high data rate transmission, and secure communication. However, deployment of cellular-connected drones over commercial LTE/5G networks still presents various challenges such as sparse coverage outside urban areas, and interference caused to the network as the UAV is visible to many towers. Commercial 5G networks can offer various features for aerial user equipment (UE) far beyond what LTE could provide by taking advantage of mmWave, flexible numerology, slicing, and the capability of applying AI-based solutions. Limited experimental data is available to investigate the operation of aerial UEs over current, without any modification, commercial 5G networks, particularly in suburban and NON-URBAN areas. In this paper, we perform a comprehensive study of drone communications over the existing low-band and mid-band 5G networks in a suburban area for different velocities and elevations, comparing the performance against that of LTE. It is important to acknowledge that the network examined in this research is primarily designed and optimized to meet the requirements of terrestrial users, and may not adequately address the needs of aerial users. This paper not only reports the Key Performance Indicators (KPIs) compared among all combinations of the test cases but also provides recommendations for aerial users to enhance their communication quality by controlling their trajectory.

==> ref.tex <==
\bibitem{variegatedLook}Narayanan, A., Zhang, X., Zhu, R., Hassan, A., Jin, S., Zhu, X., Zhang, X., Rybkin, D., Yang, Z., Mao, Z., Qian, F. \& Zhang, Z. A Variegated Look at 5G in the Wild: Performance, Power, and QoE Implications. {\em ACM SIGCOMM '21}. pp. 610-625 (2021)
\bibitem{thermal}Rochman, M., Fernandez, D., Nunez, N., Sathya, V., Ibrahim, A., Ghosh, M. \& Payne, W. Impact of Device Thermal Performance on 5G mmWave Communication Systems. {\em 2022 IEEE International Workshop Technical Committee On CQR}. pp. 1-6 (2022)
\bibitem{ALSAMHI2021102505}Alsamhi, S., Afghah, F., Sahal, R., Hawbani, A., Al-qaness, M., Lee, B. \& Guizani, M. Green internet of things using UAVs in B5G networks: A review of applications and strategies. {\em Ad Hoc Networks}. \textbf{117} pp. 102505 (2021)
\bibitem{ROVIRASUGRANES2022102790}Rovira-Sugranes, A., Razi, A., Afghah, F. \& Chakareski, J. A review of AI-enabled routing protocols for UAV networks: Trends, challenges, and future outlook. {\em Ad Hoc Networks}. \textbf{130} pp. 102790 (2022)
\bibitem{5gTracker}Narayanan, A., Ramadan, E., Quant, J., Ji, P., Qian, F. \& Zhang, Z. 5G Tracker: A Crowdsourced Platform to Enable Research Using Commercial 5g Services. {\em  ACM SIGCOMM '20 }. pp. 65-67 (0)
\bibitem{ChicagoMiami}Rochman, M., Sathya, V., Nunez, N., Fernandez, D., Ghosh, M., Ibrahim, A. \& Payne, W. A Comparison Study of Cellular Deployments in Chicago and Miami Using Apps on Smartphones. {\em WiNTECH'21}. pp. 61-68 (2021)
\bibitem{AERIQ}Maeng, S., Ozdemir, O., Güvenç, İ., Sichitiu, M., Dutta, R. \& Mushi, M. AERIQ: SDR-Based LTE I/Q Measurement and Analysis Framework for Air-to-Ground Propagation Modeling.  (2023)
\bibitem{Exhaustive}Gharib, M., Nandadapu, S. \& Afghah, F. An Exhaustive Study of Using Commercial LTE Network for UAV Communication in Rural Areas. {\em ICC '21 Workshops}. pp. 1-6 (2021)
\bibitem{SimulationsDesign}Lin, X., Wiren, R., Euler, S., Sadam, A., Määttänen, H., Muruganathan, S., Gao, S., Wang, Y., Kauppi, J., Zou, Z. \& Yajnanarayana, V. Mobile Network-Connected Drones: Field Trials, Simulations, and Design Insights. {\em IEEE Vehicular Technology Magazine}. \textbf{14}, 115-125 (2019)
\bibitem{RadioModeling}Amorim, R., Nguyen, H., Mogensen, P., Kovács, I., Wigard, J. \& Sørensen, T. Radio Channel Modeling for UAV Communication Over Cellular Networks. {\em IEEE Wireless Communications Letters}. \textbf{6}, 514-517 (2017)
\bibitem{DualNetworkControlLink}Amorim, R., Kovacs, I., Wigard, J., Pocovi, G., Sorensen, T. \& Mogensen, P. Improving Drone's Command and Control Link Reliability through Dual-Network Connectivity. {\em IEEE VTC2019}. pp. 1-6 (2019)
\bibitem{is5Gready}Bor-Yaliniz, I., Salem, M., Senerath, G. \& Yanikomeroglu, H. Is 5G Ready for Drones: A Look into Contemporary and Prospective Wireless Networks from a Standardization Perspective. {\em IEEE Wireless Communications}. \textbf{26}, 18-27 (2019)
\bibitem{Multi-tier}Sekander, S., Tabassum, H. \& Hossain, E. Multi-Tier Drone Architecture for 5G/B5G Cellular Networks: Challenges, Trends, and Prospects. {\em IEEE Communications Magazine}. \textbf{56}, 96-103 (2018)
\bibitem{5G_end2end}Festag, A., Udupa, S., Garcia, L., Wellens, R., Hecht, M. \& Ulfig, P. End-to-End Performance Measurements of Drone Communications in 5G Cellular Networks. {\em 2021 IEEE 94th Vehicular Technology Conference (VTC2021-Fall)}. pp. 1-6 (2021)
\bibitem{5GMeasure_UAV}Säe, J., Kurvi, P., Andreev, S. \& Valkama, M. Agile 5G Network Measurements: Operator Benefits of Employing Aerial Mobility. {\em IEEE Internet Of Things Magazine}. \textbf{5}, 114-119 (2022)
\bibitem{raouf2023spectrum}Raouf, A., Maeng, S., Guvenc, I., Ozdemir, O. \& Sichitiu, M. Spectrum Monitoring and Analysis in Urban and Rural Environments at Different Altitudes.  (2023)
\bibitem{wifiUav}Guillen-Perez, A., Sanchez-Iborra, R., Cano, M., Sanchez-Aarnoutse, J. \& Garcia-Haro, J. WiFi networks on drones. {\em 2016 ITU Kaleidoscope: ICTs For A Sustainable World (ITU WT)}. pp. 1-8 (2016)
\bibitem{loraUav}Ghazali, M., Teoh, K. \& Rahiman, W. A Systematic Review of Real-Time Deployments of UAV-Based LoRa Communication Network. {\em IEEE Access}. \textbf{9} pp. 124817-124830 (2021)
\bibitem{wimaxUav}Rahman, M. Enabling drone communications with WiMAX Technology. {\em IISA 2014, The 5th International Conference On Information, Intelligence, Systems And Applications}. pp. 323-328 (2014)
\bibitem{zhangInfocom}Narayanan, A., Rochman, M., Hassan, A., Firmansyah, B., Sathya, V., Ghosh, M., Qian, F. \& Zhang, Z. A Comparative Measurement Study of Commercial 5G mmWave Deployments. {\em IEEE INFOCOM}. pp. 800-809 (2022)
\bibitem{kthBvlos}Ozger, M., Vondra, M. \& Cavdar, C. Towards beyond Visual Line of Sight Piloting of UAVs with Ultra Reliable Low Latency Communication. {\em IEEE GLOBECOM}. pp. 1-6 (2018)

